An Independent Implementation of Quantum Machine Learning Algorithms in Qiskit for Genomic Data

In this paper, we explore the power of Quantum Machine Learning as we extend, implement and evaluate algorithms like Quantum Support Vector Classifier (QSVC), Pegasos-QSVC, Variational Quantum Circuits (VQC), and Quantum Neural Networks (QNN) in Qiskit with diverse feature mapping techniques for genomic sequence classification.

==> body.tex <==
\section{Introduction}
 {\color{red} Perhaps NTN and cognitive (queuing) aspects}

LEO satellites, due to their orbital mobility, maintain intermittent but predictable communication with ground terminals and devices~\cite{razmi2021board}. Li~\cite{Jian2020} explores seamless handovers for optimal LEO links. Despite these initiatives, end-users in new applications demand shorter wait times for timely data collection and real-time status updates with reasonable QoS. Figure~\ref{fig:first} illustrates LEO buffer dynamics, queuing delays, and challenges from propagation, transmission delays, affecting overall QoS. Understanding the LEO buffering challenge is crucial for optimizing uplink and downlink channels and improving QoS~\cite{Zlatanov14}. Queuing mechanisms depend on various factors, including satellite capacity, channel conditions, buffer size, data traffic arrivals/departures at LEOs, and overall data flow dynamics. A thorough queuing analysis can offer insights for load balancing and cooperation in LEO constellations. However, existing work, including~\cite{Jian2020, razmi2021board}, has not deeply analyzed LEO queuing mechanisms, leaving their impact poorly understood in the literature.
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{setup1.png}
    \caption{Cognitive Queuing over LEOs by exchanging the queue occupancy and early signaling near full buffers over erroneous uplinks and downlinks.}
    \label{fig:first}
\end{figure}
% \begin{itemize}
%     \item LEO constellations $\to $ single orbit
%     \item Handover: we do not consider it in this paper
%     \item Queuing: Arrival processes/Departure processes (beamwidth, speed of LEO, density of IoT devices, density of ground terminals, etc)
%     \item Collaboration between adjacent LEOs
%     \item Adjacent LEOs exchanges their queues status (distributed control)
%     \item uplink/downlink performance improvements
% \end{itemize}


\subsection{Relatedworks}
This work is closely related to the recent analyses presented in~\cite{chiariotti2020information, soret2020latency, soret20215g}. %In~\cite{chiariotti2020information, soret2020latency}, the authors explore Age of Information (AoI) based on queueing delay in a comparable LEO setup, where satellites forward data from IoT devices to a ground terminal. Another use case of 5G offloading and backhauling in the absence of mobile infrastructure is proposed in~\cite{soret20215g}. However, all these studies assume M/M/1 queue models, failing to capture the time-varying dynamics inherent in LEO links due to factors like fading, Doppler, and rain.

Earlier works in~\cite{957168, 1040571, tan2014analysis} provide additional context. Chen \textit{et. al.}\cite{957168} employ a Markov chain to study queueing dynamics in a single satellite setup, while Yeo~\cite{1040571} simulates end-to-end delay in LEO satellite constellations without considering queue figures. Tan \textit{et. al}\cite{tan2014analysis} analyze the system by modeling the average number of inter-satellite links, considering Poisson-distributed incoming traffic but overlooking the actual queuing process.

Zhu \textit{et. al.}\cite{zhu2018performance} investigate intermittent satellite connectivity in LEO constellations using a two-state Markov model, determined by Line of Sight (LoS) times. However, they do not consider queue occupancy and the underlying queuing process. In~\cite{speidel2018striking}, when quantifying the delay of queuing in satellite networks and its impact on the transmission control protocol (TCP)~\cite{Pokhrel2019Mob}, simulations are used to predict the optimal buffer size, focusing on packet loss during TCP data transfer rather than the underlying causes of loss and queueing. This approach falls short in capturing the required system dynamics for time-varying LEO channel states in downlinks to ground terminals.


\subsection{Contributions}
Our primary contribution in this paper is the following.
\begin{enumerate}
\item \emph{We create a new cognitive model of queueing for LEO-based IoT data network that works in cooperative settings.} 
\end{enumerate}



\section{Network Settings and Scenario}


We consider a single orbit LEOs network illustrated in Fig.~\ref{fig:first}, where adjacent LEO satellites share a common objective, such as optimizing data collection from ground sensors and ensuring optimal downlink transmissions to ground terminals.

In this network scenario, $n\in{1,2,\dots,N}$ LEO satellites move at a constant speed of $v$ km/sec, collecting data from ground IoT sensors via beamforming on their uplink channels (refer to Fig.~\ref{fig:first}). At any given time, uplink data from all sensors is directed through the same LEO unless its buffer is full. Buffer loss occurs when the buffer is full, leading to uplink transmission failures and data loss due to both buffer overflows and poor channel conditions.

As depicted in Fig.~\ref{fig:first}, the $(n-1)^{th}$ LEO can be continuously informed of the queue occupancy status, $Q_n(t)$, of the $n^{th}$ LEO. Consequently, the $(n-1)^{th}$ LEO can better prepare for additional data collection by draining its buffer. Under favorable downlink channel conditions, LEO buffers can be promptly drained via transmission to the ground terminal. However, unsuccessful downlink transmissions occur when channel conditions are poor.

For instance, due to transient buffering and varying channel conditions, if one LEO fails (buffer overflows or the channel is erroneous) to meet its uplink/downlink requirements, the adjacent LEO can be informed for potential support. Therefore, adjacent LEOs can be seen as cooperative in achieving a common goal through the exchange of buffer occupancy and dynamics, while also operating non-cooperatively to maximize their individual utilities through efficient resource allocation.
 



\subsection{Analytic System Model}\label{sec:sysmodel}
%\subsection{Geometric Model}
Suppose that a LEO satellite at an altitude $h$ has a ground speed of $v$. We consider a time slotted system for communications and the duration of the time slot is denoted by $T_{\rm s}$. Then, the ground area per time slot becomes
\be 
A_{\rm s} = v T_{\rm s} D,
\ee 
where $D$ represents the beamwidth footprint, for an approximation. Here, we consider a spherical cap of coverage on Earth's surface, which can be covered by a spot beam. Accordingly, $D$ is the spherical cap base diameter and can be computed as follows
\begin{equation}
    D = 2R_\oplus\sin\varphi_\mathrm{m},
\end{equation}
where $R_\oplus$ is Earth's average radius and $\varphi_\mathrm{m}$ is the maximum zenith angle that the satellite beamwidth can extend as follows~\cite{9509510}:
\begin{equation}
\varphi_\mathrm{m}(\psi) =
\begin{cases}
    \asin\left(\frac{1}{\alpha}\sin\frac{\psi}{2}\right) - \frac{\psi}{2},  &\mbox{if $\psi \le 2\asin\alpha$} \\
    \acos\alpha,  &\mbox{if $\psi>2\asin\alpha$} \\
\end{cases}
\end{equation}
where $\psi$ is the satellite beamwidth and $\alpha = R_\oplus/(R_\oplus + h)$.

% \begin{figure}[t]
% \begin{center}
% \includegraphics[scale=0.5]{LEO.pdf} 
% \end{center}
% \caption{A coverage area of LEO with a spot beam.}
%         \label{Fig:LEO}
% \end{figure}
The number of IoT devices on the ground is assumed to follow a homogeneous Poisson process with parameter $\kappa> 0$ so that the probability that there are $M = m$ devices in the sphere cap per time slot becomes
\be 
\Pr(M = m) = \frac{ (\kappa A_{\rm s} )^m}{m!} e^{- \kappa A_{\rm s}}.
\ee 

Considering these system aspects, we have adopted a modular approach for building our system model. The structural overview of our analytic model, which comprises seven different components, is shown in Fig.~\ref{fig:block}. While some of these modules are developed based on queuing theory~\cite{medhi2002stochastic} and channel models~\cite{9509510}, others are newly developed in the context of this work. Furthermore, to the best of our knowledge, the proposed modular analytic model is the first method for capturing queuing dynamics over LEO, which is developed by combining all of seven components into a consolidated system model. Fig.~\ref{fig:block} depicts the dependencies between components of the proposed system model. Each component's system expressions are developed based on the assumption that the outputs from the other components (as inputs to the component) are readily available. In the following, we explain each of the seven modules of Fig.~\ref{fig:block} in details.

\subsection{Packet Arrival and Service Process}
It is assumed that a device in the ground area per time slot becomes active with probability $p_{\rm a}$. Then, letting $\Lambda = \kappa A_{\rm s}$, the number of active devices transmitting their data packets follows a Poisson distribution with parameter $p_{\rm a} \Lambda = p_{\rm a} \kappa v D T_{\rm s}$. That is, the number of arrivals, denoted by $U$, within time slot has the following distribution
\be 
\Pr(U = m) = \frac{ (\lambda T_{\rm s} )^m}{m!} 
e^{- \lambda T_{\rm s}};\\
\lambda = p_{\rm a} \kappa v D (1-p_{\mathrm{up}}),
\label{eq:PASP}
\ee 
where $p_{\mathrm{up}}$ is the probability that the uplink transmission fails due to channel impairments, such as shadowing, rain fading, etc (see  Sec.~\ref{sec:pup-pdp} for details). 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.3]{blockdiag.png}
    \caption{Interrelationships between different components.}
    \label{fig:block}
\end{figure}
Each LEO has a buffer where it stores the received packets in order to relay them to a ground terminal. The number of packets that can be transmitted to a ground terminal during a slot interval becomes
\be 
S =  \left\lfloor \frac{T_{\rm s} W \log_2 (1+ \gamma )}{L} \right\rfloor
\in \{0,1,\ldots\},
\ee 
where $L$ represents the size of packets in bits, $W$ denotes the downlink bandwidth from a LEO to a ground terminal in Hertz, and $\gamma$ represents the signal-to-noise ratio (SNR). Since the SNR varies, it can be modeled as a random variable that has the following distribution:
\begin{align} 
\label{eqn:GaussianSNR}
\Pr(S = k) 
& = \Pr \left( 
\frac{k L}{T_{\rm s} W} \le 
\log_2 (1+ \gamma) < \frac{(k+1) L}{T_{\rm s} W}
\right) \cr 
& = \Pr \left(
2^{\frac{k L}{T_{\rm s} W}} - 1 \le \gamma 
< 2^{\frac{(k+1)L}{T_{\rm s} W}} - 1 
\right) . 
\end{align} 
Thus, for a given distribution of SNR, the distribution of $S$ can be found.


\subsection{Modeling Queuing Dynamics}
As mentioned, we consider that the LEO's queue sees packet arrivals according to a Poisson process at a rate $\lambda$. Given Poisson arrivals, we can consider the first-in first-out (FIFO) service order and the queue follows the $M/G/1/K$ dynamics. The distribution of the service rate of this process can be computed as in \eqref{eqn:GaussianSNR}. Since the LEO's buffer capacity is $K$ packets (finite), the queue occupancy for all $0 < \lambda < \infty$ is a stationary ergodic process and, there exists a stationary probability of buffer overflow, $p_b$, referred to as the blocking probability. Next we compute
\begin{align*}
a_i &= \Pr \left( i \; \mbox{packets arrive during a service time} \right) \\
&=\int_{0}^{\infty} e^{-\lambda u} \frac{(\lambda u)^i}{i!}dF(u)\nonumber\\ %dF_G(u) %= \bE \left[ e^{-\lambda G} \frac{(\lambda G)^i}{i!} \right] \nonumber \\ 
&=\textcolor {black}{\sum_{k} \Pr(S= k) e^{-\lambda k T_s} \frac{(\lambda k T_s)^i}{i!}},
\end{align*}
where $i$ represents the number of packets arriving.

Let $\tilde{Q}_i$ be the number of packets in the buffer when the $i$-th packet is served. Then, $\{\tilde{Q}_i, i \geq 1\}$ is a Markov chain whose transition probabilities depend only on $a_i$, $i\geq 0$. Considering \[{\bx = (x_0, \dots, x_{K-1})}\] as the probability vector of the chain $\{\tilde{Q}_i, i \geq 1\}$, where $x_i$ is the (stationary) probability that a serving packet leaves the LEO queue with $i$ packets (i.e., ${0 \leq i \leq K-1}$) behind. We compute $\bx$ by a standard method using $a_i$~\cite{medhi2002stochastic}. Also the probability that a packet leaves the LEO buffer empty (i.e., $\lim_{k \rightarrow \infty} \Pr(\tilde{Q}_k = 0$) exists at $x_0$.

\subsection{Estimating Traffic Intensity}
At any point in time, denoting by $\eta_j$, $0 \leq j \leq K$, the probability that there are $j$ packets in the LEO queue, we have
\begin{align}
\label{eqn:nuj}
\eta_j &= \bE\Big[\frac{x_j}{x_0+\frac{\lambda} {S}}\Big], \quad 0 \leq j \leq K-1, \\
&=\sum_{s\in K}\Pr(S = s)\frac{sx_j}{sx_0+{\lambda T_s}}\nonumber
\end{align}
\begin{align}
\label{eqn:nujk}
\eta_K &= 1 - \bE\Big[\frac{1}{x_0+\frac{\lambda} {S}}\Big]\\
&=1-\sum_{s\in K}\Pr(S = s)\frac{s}{s x_0+{\lambda T_s}}.  \nonumber
\end{align}
%With relevant insights from~\eqref{eqn:nuj} and~\eqref{eqn:nujk}, we define $\varrho$  as the expected traffic intensity of the individual LEO queuing process and use it as a tool to analyze the equilibrium of multiple LEO queues.
% \begin{eqnarray}
% \bE\left[\frac{\lambda} {S}\right]=\begin{cases}
%     \frac{\lambda} {\bE\left[S\right]}, & \text{if $j=0$}.\\
%     \sum_{j}  \frac{\lambda T_s}{ j}\Pr(S = j), & \quad 0 < j \leq K-1.\nonumber
%   \end{cases}
% \end{eqnarray}
   
% {\color{red} check the above equation:
% $  \bE\left[\frac{\lambda} {S}\right]$ has to be
% $$
%     \bE\left[\frac{\lambda} {S}\right] = \sum_{j \in K}  \frac{\lambda T_s}{ j}\Pr(S = j).
% $$
% However, since $j$ can be  $0$,  $\bE\left[\frac{\lambda} {S}\right] =\infty$.
% Thus, it might be 
% $$
%  \bE\left[\frac{\lambda} {S}\right] \Rightarrow 
%   \frac{\lambda} {\bE\left[S\right]}
%  $$
% }


\subsection{Buffer Overflow and Throughput Analysis}


We know that the number of packets in the queue viewed by the $i$-th arriving packet is $\hat{Q}_i$.
Because Poisson arrivals observe time averages, the likelihood that an arriving packet sees $j$ packets in the queue is equal to the probability that $j$ packets exist in the queue. 
\begin{equation*}
\label{eqn:Qhatj} 
\lim_{n \rightarrow \infty} \Pr(\hat{Q}_i = j) = \eta_{j}, 
\end{equation*}
therefore,
\begin{equation}
\label{eqn:pb}
p_b = \lim_{n \rightarrow \infty} \Pr(\hat{Q}_i = K) = \eta_{K}. 
\end{equation}
\begin{figure}\captionsetup{font=footnotesize,labelfont=footnotesize,justification=raggedright,singlelinecheck = false}
	\begin{subfigure}{0.4\linewidth}
		%\caption{Uplink}
		\includegraphics[width=\linewidth]{Diagram1.eps}
	\end{subfigure}
	\begin{subfigure}{0.4\linewidth}
		%\caption{Downlink}
		\includegraphics[width=\linewidth]{Diagram2.eps}
	\end{subfigure}
	\centering
	\caption{A representation of the satellite-centric geometric model utilized in this analysis for uplink (left) and downlink (right) communications.}
	\label{Fig_Schematic}
\end{figure}

A served packet from LEO to a ground terminal is successful with probability $(1-p_\mathrm{dn})$, where $p_\mathrm{dn}$ is the probability of packet loss in the downlink channel (computed later in Sec.~\ref{sec:pup-pdp}).  
Since the average rate at which packets gets into the LEO buffer is determined  by the probability  $\lambda (1-p_b)$,
the average packet reception rate at a ground terminal, denoted by
$\bar S$, is given by,% Since the queue length process is stable, the rate at which packets are served (i.e., leave the queue) is also equal to $\lambda (1-p_b)$. Hence, the throughput, $S$, can be estimated as $\lambda (1-p_b) (1-p_c)$. In particular, the arrival rate $\lambda$ satisfies
\begin{equation}
\label{eqn:lambda}
%\lambda = \frac{\Theta}{1-\tilde{q}} = \frac{\Theta}{(1-p_b)(1-p_w)}. 
\bar S =\lambda{(1-p_b)(1-p_\mathrm{dn})}. 
\end{equation}

Using the ideas from~\eqref{eqn:nuj},\eqref{eqn:nujk} and~\eqref{eqn:lambda}, we define the expected traffic intensity 
\be
\varrho=\frac{\lambda T_s}{\bar S}
\ee   
of the individual LEO queuing process and use it as a tool to analyze the system equilibrium ($\varrho^*$, $p_b^*$) and understand the stability of the proposed cooperative queuing framework (Sec.~\ref{sec:LEOs}).

\subsection{Queuing and End-to-End Delay}
 The round trip data collection delay from \textit{IoT sensors through LEO to ground terminal} can be estimated as~\cite{Pokhrel2019Mob} 
\[T = T_d + T_Q,\] 
where $T_Q$ is the queuing delay at the LEO (waiting plus service time), and $T_d$ is the total propagation delay in the uplink and in the downlink channel, $T_d=T_\mathrm{up}+T_\mathrm{dn}$.

Also the rate at which packets enters into the LEO buffer is governed by $\lambda (1-p_b)$. Therefore, the queuing delay at LEO, $T_Q$, can be computed using Little's law as
\begin{eqnarray}
T_Q = \frac{\bE[Q]} {\lambda (1-p_b)}
\end{eqnarray}
where 
\[\bE[Q] = \sum_{j=1}^K j \eta_j.\] 
is the expected packets in the LEO queue.
% \begin{remark}[\textit{Residual Time}]
% The remaining time until the next transition epoch in the channel state Markov chain is the residual service time as seen by the $i$-th arriving packet. Due to Poisson arrivals, the residual time is uniformly distributed over the interval and can be estimated as $U_{[0,T_s]}$. 
% If the $i^{th}$ arriving packet sees the queue empty, then the residual time is $U_{[0,T_s]}$, else if the arrival sees packets in the LEO queue, we have the following assumption. We assume that when an arriving packet finds at least one packet in the LEO queue, the residual service time observed by the packet is independent of the precise number of packets found in the queue and equal to the stationary residual service time.
% \end{remark}

% {\color{red}
% If 
% \be 
% \Pr(S = 0) = \Pr \left(\gamma 
% < 2^{\frac{(k+1)L}{T_{\rm s} W}} - 1 
% \right) = \exp(- \mu T_{\rm s}) ,
% \ee 
% as
% $T_{\rm s} \to 0$, we have M/M/1 queue

% In general, we may have M/G/1 queue

% }
\subsection{Satellite Channel Model}



\label{sec:channel model}
Unlike its terrestrial counterpart, the vast proportion of a satellite communications occurs in free-space and a small portion only experiences rain fading (especially for frequencies above 10~GHz)~\cite{1141845} and shadowed small-scale fading~\cite{1623307}. Hence, the satellite channel power can be modeled as follows:
\begin{equation}\label{Eq_Channel}
    \vert g(\varphi)\vert^2 = l(\varphi)\zeta(\varphi)\chi(\varphi)~,
\end{equation}
where $\varphi$ is the Earth-centered zenith angle between the satellite and ground terminal, and $l$ is the free-space-gain as follows:
\begin{equation}
    l(\varphi) = \frac{l_\mathrm{o}}{R_\oplus^2 + (R_\oplus+h)^2-2R_\oplus(R_\oplus+h)\cos\varphi}~.
\end{equation}
Here, $l_\mathrm{o}=c^2/(4\pi f)^2$ is the path-gain constant,
where $c$ is the speed of light and $f$ is the center frequency. On the other hand, $\zeta$ in \eqref{Eq_Channel} is the excess path-loss assumed to comprise two states; line-of-sight (LoS) and non-line-of-sight (nLoS), represented by a mixed log-normal random variable as follows:
\begin{align}
    \zeta \sim p_{\LoS}(\varphi)\mathcal{LN}(\mu_{\LoS},\sigma_{\LoS}) + p_{\nLoS}(\varphi)\mathcal{LN}(\mu_{\nLoS},\sigma_{\nLoS})~,
\end{align}
where $\mu_{\LoS}, \sigma_{\LoS}, \mu_{\nLoS}, \sigma_{\nLoS}$ are the LoS and nLoS power average and standard deviation. The probability of LoS determines the state which in turn is dependent on the zenith angle obtained as follows~\cite{9509510}, $p_\mathsf{LoS} = \exp[-\beta\sin\varphi/(\cos\varphi - \alpha)]$ where $\beta$ is a constant that relies on the propagation environment. In addition, we donate the average rain power attenuation $\chi$ which is a function of the elevation angle and by extension the Earth-centered zenith angle as follows:
\begin{equation}\label{Eq_Rain}
\chi\mathrm{[dB]} = aR^b (h_\mathrm{R} - h_\mathrm{s}) c_{\rm pl}
\left[\sqrt{\frac{\sin^2\varphi}{(\cos\varphi - \alpha)^2}+1}\right],
\end{equation}
where $c_{\rm pl}$ is the path-length reduction constant, $a$ and $b$ are parameters that depend on the frequency~\cite{1141845}, $R$ is the average rain rate, and $h_\mathrm{R}$ and $h_\mathrm{s}$ are the rain height and ground terminal height respectively. The derivation of \eqref{Eq_Rain} is in Appendix~\ref{App_A}.

\subsection{Transmission Failures}
\label{sec:pup-pdp}

IoT devices are assumed to  transmit signals with a constant transmit effective isotropic radiated power (EIRP), denoted by $P_\mathrm{t}$, without power control. On the other hand, the LEO satellite has a receiving antenna with a dynamically varying beamwidth~\cite{9684552}, denoted by $\psi_\mathrm{up}$, illustrated in Fig.~\ref{Fig_Schematic}. The gain of the LEO receive antenna, denoted by $G_\mathrm{r}$, is assumed to be ideal and is controlled by the beamwidth, i.e. a narrow beamwidth results in a highly directional gain. The received power at the LEO is obtained as follows:
\begin{equation}
    \rho_\mathrm{r} = P_\mathrm{t} G_\mathrm{r}(\psi_\mathrm{up})\vert g(\varphi_\mathrm{t})\vert^2,
\end{equation}
where $\varphi_\mathrm{t}$ represents the Earth-centered global zenith of a typical ground IoT device. Accordingly, the average uplink probability of transmission failure, denoted by $p_\mathrm{up}$, is obtained as the probability that the SNR, $\gamma_\mathrm{up}$, is lower than a threshold, $\gamma_\mathrm{o}$, as follows:
\begin{align}
    &p_\mathrm{up} = \Pr(\gamma_\mathrm{up}<\gamma_\mathrm{o}) \nonumber\\&= p_\mathrm{a}\Lambda\int_{0}^{\varphi_\mathrm{m}(\psi_\mathrm{up})} F_\zeta\left(\frac{\gamma_\mathrm{o}N_\mathrm{s}}{\rho_\mathrm{t} G_\mathrm{r}l(\varphi_\mathrm{t})\chi(\varphi_\mathrm{t})}\right)f_\mathcal{A}(\varphi_\mathrm{t}) {\rm d} \varphi_\mathrm{t},
    \label{eqn:17}
\end{align}
where $N_\mathrm{s}$ is the noise floor at the LEO receiver.

In the downlink, the LEO is assumed to transmit at a constant power, denoted by $\rho_\mathrm{t}$, which corresponds to the output of its repeater. Moreover, the LEO transmitter gain $G_\mathrm{t}$ is similarly dynamically controlled by varying the downlink beamwidth $\psi_\mathrm{dn}$ as illustrated in Fig.~\ref{Fig_Schematic}. On the other hand, the ground terminals are assumed to have a constant gain, denoted by $G_\mathrm{g}$. As a result, the received power at the ground terminal is obtained as follows:
\begin{equation}
    \rho_\mathrm{g} = \rho_\mathrm{t} G_\mathrm{t}(\psi_\mathrm{dn}) G_\mathrm{g}\vert g(\varphi_\mathrm{g})\vert^2,
\end{equation}
where $\varphi_\mathrm{g}$ represents the Earth-centered global zenith of a typical ground terminal. The probability of downlink transmission failure, $p_\mathrm{dn}$, is obtained as the probability that the downlink SNR, $\gamma_\mathrm{dn}$, is lower than a threshold, $\gamma_\mathrm{o}$, as follows:
\begin{align}
    &p_\mathrm{dn} = \Pr(\gamma_\mathrm{dn}<\gamma_\mathrm{o}) \nonumber\\ &=  \int_{0}^{\varphi_\mathrm{m}(\psi_\mathrm{dn})} F_\zeta\left(\frac{\gamma_\mathrm{o}N_\mathrm{g}}{\rho_\mathrm{t} G_\mathrm{t}G_\mathrm{g}l(\varphi_\mathrm{g})\chi(\varphi_\mathrm{g})}\right)f_\mathcal{A}(\varphi_\mathrm{g}) {\rm d} \varphi_{\rm g},
    \label{eqn:18}
\end{align}
where $N_\mathrm{g}$ is the noise floor at the ground terminal. %The details of Equations~\eqref{eqn:17} and~\eqref{eqn:18} are provided in Appendix~\ref{App_B}.

%\subsection{Throughput Model}




% \subsection {Markovian Channel Modeling}
% \begin{figure}[h]
% \centering
% \begin{tikzpicture}{shorten >=1pt,node distance=10cm,on grid,auto}
% \node[state] (q_1) {$GOOD$}; 
% %\node[state] (q_1) [ right=of q_1] {$G$}; 
% \node[state] (q_2) [ right=of q_1] {$BAD$}; 
% %\node[state] (q_3) [ right=of q_2] {$n+1$}; 
% %\node[state,draw=none] (q_4) [ right=of q_3] {}; 
% \path[->] 
% %(q_0) edge [bend right] node [below left] {$\frac{1-p_{we}}{n-1}$} (q_1)
% %(q_1) edge [bend right]node [above right] {$\frac{n-1}{n}$} (q_0) 
% (q_1) edge [bend right] node [below] {$1-{\bar p_g}$} (q_2)
% edge [loop below] node {${\bar p_g}$} (q_2)
% (q_2) edge [bend right]node [above] {$1-{\bar p_b}$} (q_1) 
% %(q_2) edge [bend right] node [below right] {$\frac{1-p_{we}}{n+1}$} (q_3)
% edge [loop above] node {${\bar p_b}$} (q_1);
% %$(q_3) edge [bend right]node [above right] {$\frac{n+1}{n+2}$} (q_2); 
% %(q_3) edge [bend right] node [below left] {$\frac{1-p_{we}}{n+2}$} (q_4)
% %(q_4) edge [bend right]node [above right] {$\frac{n+2}{n+3}$} (q_3) ;
% \end{tikzpicture}
% \caption{Markovian state transition diagram for tracking erroneous channel (due to contention, collision, fading etc.).\label{fig:state-transition}}
% \end{figure}
%  The stationary channel state transition probabilities of the Markovian channel model shown in Fig.\ \ref{fig:state-transition} can be computed as

% \begin{eqnarray}
% \label{eq:active-channel}
% \lefteqn{{\mathbb P}(\mbox{Channel stays in bad state})}&& \nonumber \\
% &&={\bar p_b}= , \;\;\;\mbox{and} \\
% \lefteqn{{\mathbb P}(\mbox{Channel stays in good state})}&& \nonumber \\
% &&={\bar p_g}=  \;\;\; 
% \end{eqnarray}



%\begin{equation}
%    G_\mathrm{t} = \frac{1}{1 + \cos\frac{\psi}{2}}~,
%\end{equation}


% \begin{figure*}
% \begin{align}
%     &\Pr (S=k)  =  \Pr \left(2^{\frac{k L}{T_{\rm s} W}} - 1 \le \gamma < 2^{\frac{(k+1)L}{T_{\rm s} W}} - 1 \right) = \Pr( \gamma < 2^{\frac{(k+1)L}{T_{\rm s} W}} - 1 )- \Pr( \gamma < 2^{\frac{kL}{T_{\rm s} W}} - 1 ) = \nonumber\\
%     &\int_{0}^{\varphi_\mathrm{m}}\left(1 - F_\zeta\left[\frac{(2^{\frac{kL}{T_{\rm s} W}} - 1)N}{\rho_\mathrm{t} G_\mathrm{t} G_\mathrm{r}l(\varphi_\mathrm{o})\chi(\varphi_\mathrm{o})}\right]\right)f_\mathcal{A}(\varphi_\mathrm{o})\mathrm{d}\varphi_\mathrm{o} - \int_{0}^{\varphi_\mathrm{m}}\left(1 - F_\zeta\left[\frac{(2^{\frac{(k+1)L}{T_{\rm s} W}} - 1)N}{\rho_\mathrm{t} G_\mathrm{t} G_\mathrm{r}l(\varphi_\mathrm{o})\chi(\varphi_\mathrm{o})}\right]\right)f_\mathcal{A}(\varphi_\mathrm{o})\mathrm{d}\varphi_\mathrm{o},
% \end{align}
% \end{figure*}

%{\color{red}
%\be  
%\Pr (S=k) = \Pr( \gamma < 2^{\frac{(k+1)L}{T_{\rm s} W}} - 1 )
%- \Pr( \gamma < 2^{\frac{kL}{T_{\rm s} W}} - 1 ). \ \ 
%\ee 
%}


% \subsection{Queuing Model}

% Arrival process: Poisson process, $\zeta$

% \subsection{Departure process}
% $$
% R = W \log_2 (1+ SNR(t) )
% $$

% M/G/1

% speed of LEO ... 

 \section{Adaptive Cooperation between LEOs}
\label{sec:LEOs}

\subsection{Cross Queue Analysis}
\label{subsubsec:compute-h}

With slight abuse of notations, let $\lambda_{n}$ denote the arrival rate of packets into the $n^{th}$ LEO buffer of capacity, denoted by
$K_n$, from the IoT devices. Then, in the steady state, the ratio of the arrival rate packets 
into the queue to the total arrival rate into 
all LEOs buffers is represented by the probability $\cR_n$ that the packet belongs to the buffer of capacity $K_n$, having the queue occupancy state $Q_n$, i.e., 
\begin{eqnarray}
\cR_n = \frac{\lambda_{\rm n}}{\sum_n\lambda_{n}}
 \approx \frac{\bE[Q_n]}{\sum_n \bE[Q_n]}
 \approx \frac{\frac{\bar S_n }{(1-p_{dn,n})} }{ {\sum_n \frac{\bar S_n} {(1-p_{dn,n})}} },
\label{eq:h}
\end{eqnarray} 
where $\bar S_n$ is the average
packet reception rate from the $n^{th}$ LEO buffer to a ground terminal and $p_{dn,n}$ is the corresponding downlink transmission failure in the channel. The approximation in~\eqref{eq:h} results from that the delay experienced by all packets is due to LEO queuing and therefore data packets through the same LEO experiences the same delay.

\subsection{Buffer-Aided Adaptive Cooperation (BAAC)}

For our cooperative approach, rather than starting with the buffer of capacity $K_n$ for the $\rm n^{th}$ LEO a priori, we solve the equations \eqref{eq:PASP}-\eqref{eq:h} with $\cR_n$ as a constant and get convergent results. This is the proposed signaling and co-operation between LEOs refer to as \textit{BAAC algorithm}. Assuming practical inter-satellite links and cooperative communication, BAAC can be readily handled by a software patch at the LEO, and it would be compatible with existing LEO standards and communication protocols. See the details of BAAC in Algorithm~\ref{shCHalgorithm}. At the LEO buffers, the necessary throughput ratio required for the data collection can be achieved by using one of the two ways below:

\begin{enumerate}
    \item [a)]  \textit{Performance solution.} Set a large LEO buffer and block the packets arriving at the LEO buffer by probability $p_b(\cR_n(t))$. Another method to implement this solution along the lines is to activate IoT devices in the ground area per time slot with probability $1-p_b(\cR_n(t))$.
    \item [b)] \textit{Latency-sensitive solution.} With an objective to minimize $\min\; (Q_n(t)-\beta K_n)^2$, our goal is to always attain buffer occupancy  $Q_n(t) = \beta K_n$; where $0<\beta<1$.
\end{enumerate}


\begin{algorithm}[t]
\caption{BAAC Algorithm at each LEO}
\label{shCHalgorithm}
\begin{algorithmic}[1]
\Procedure{Setup} {}\\
Set desired performance ratio of each LEO ($\cR_n^*$), Buffer Capacity ($K_n$)
\EndProcedure
\Procedure{BAAC Update} {}
\While{$((Q_n(t)-\beta K_n)^2>tol)$ }
\If {$({\cR_n(t)<\cR_n^*})$ }
$p_b(t)=0.0$
\Else \;$p_b(t)=1.0$
\EndIf
\Procedure {Observe LEO Queue}{}\\
\hspace{15 mm} Renew $\cR_n$ and $Q_n$
\EndProcedure
\EndWhile
\EndProcedure
\end{algorithmic}
\end{algorithm}


The blocking probability $p_b(t)$ should adjust when the LEO satellite channel degrades or packet arrival rates vary over time.
Assume that the LEO network is stable at one time slot and that the performance ratio is at the acceptable level closer to the desired $\cR_n^*$, then, when the magnitude of channel loss ($p_{up}(t)$ or $p_{dn}(t)$) changes, the previous value of admission probability causes performance to deviate from the intended value, and the new value $\cR_n(t)$ will be mirrored at the LEO queue. By continuously renewing the value of $p_b(\cR_n(t))$, our BAAC algorithm intelligently exploits this deviation and steer the system dynamics to the target $\cR_n^*$. The BAAC keeps track of the transient LEO queue occupancy $Q_n(t)$ (observable locally at a LEO) and always guarantee that it maintains the required total capacity $\beta K_n$ on average.


% \subsection{Mathematical Interpretation of BAAC Algorithm}
% When there are multiple data flows from different devices, we can use the following loss formula of small buffers:
% \begin{eqnarray}
% p_b(\cR_n(t))=\Big(\frac{\lambda_{n}(t)}{S_n(t)}\Big)^{c\cR_n^*K}
% \label{eqn:vbs}
% \end{eqnarray}
% where $\lambda_{n}(t)$ is the arrival rate at the AP, $S_n(t)$ is the WiFi service rate, and the factor $c\cR_n^*K$ is the buffer space.
% buffer states can be exchanged

% \subsection{Convergence and Stability of BAAC}
% \label{sec:stability}
% Using the proposed BAAC algorithm, there are numerous options for selecting the buffer size, $\beta K_n$~\cite{mckeown2019sizing}. For example, in a large buffer scheme, we can allow the LEO buffer size to be proportional to the number of flows (this is the traditional rule of thumb), which states that the buffer size should be equal to the channel bandwidth-delay product. In sharp contrast, we can adopt a fixed Drop Tail buffer and exploit statistical multiplexing in a small buffer scheme to keep overflow loss minimal. %Another case for an intermediate buffer size selection (a major departure from the traditional rule of thumb) with several data flows in the the buffer suggests~\cite{mckeown2019sizing} \[\beta K_n:=\frac{ bandwidth-delay \;product}{\sqrt{number\; of\; flows}}.\]


% With the buffer sizing, to understand the convergence and stability aspects under the BAAC algorithm one can apply the theories from dynamical systems. For instance, we can see if the system is locally stable under BAAC. Local stability with buffer sizing is reasonably studied well using dynamical systems; see~\cite{mckeown2019sizing} and the references therein. However, when the system is unstable, we need to quantify the magnitude of the traffic oscillations. Moreover, when the system is locally stable, the data collection flows are completely unsynchronized, but when there are oscillations, there is often some degree of synchronization. The more significant the oscillations, the greater the degree of synchronization. %As a result, we need to rank the various buffer-sizing recommendations by the proposed BAAC.\footnote{The effect of oscillations on the system performance for the network setup considered in this paper requires detailed theoretical studies and will be investigated in the future.}

% Oscillations can be better understood with extensive simulations, which also provides ideas to study the convergence and stability aspects of the BAAC algorithm. For example, every BAAC recommended buffer size can be evaluated with simulations first. We have conducted simulations to study the oscillations and convergence aspects of the system dynamics with BAAC. In particular, we apply a simple stability check approach by utilizing the developed empirical framework. First, we find the equilibrium point ($\varrho^*, p_b^*$) given the uplink/downlink channel condition and $\beta K$; we then use simulations to see if the system dynamics with BAAC is oscillating and locally stable around this equilibrium point or not. 




%\bibliographystyle{IEEEtran}
%\bibliography{VBandPaper}

%\appendix


\begin{table}[t]
	\caption{Simulation Parameters}
	\centering
	\begin{tabularx}{3.49in}{l l l}
		\hline\hline \\[-1.5ex]
		Symbol & Value &Definition \\
		\hline\\ [-1.5ex]
		$R_{\tinyEarth}, h$ & 6371km, 1200km & Earth's radius \& Sat altitude \\
		$f_\mathrm{up},f_\mathrm{dn}$ &17.7GHz, 27.5GHz &Uplink \& Downlink center frequency \\
		$\psi_\mathrm{up},\psi_\mathrm{dn}$ &30$^\circ$-60$^\circ$, 90$^\circ$ & Uplink \& Downlink Beamwidth \\
		$\rho_\mathrm{t}G_\mathrm{t},P_\mathrm{t}$ & 30dBm, 40dBm & Sat \& IoT device EIRP \\
		$G_\mathrm{r}$, $G_\mathrm{g}$ & 30dB, 30dB & Sat \& terminal receive gain \\
		$D, \gamma_{\mathrm{o}}$ & 1\%, 5dB & User duty cycle, target SINR \\
		%$\beta$ &0.31 &LoS probability parameter \\
		$\mu_{\LoS}, \mu_{\nLoS}$ &0dB, 20dB &LoS/nLoS excess path-loss mean \\
		$\sigma_{\LoS}, \sigma_{\nLoS}$ &0.1dB, 8dB &LoS/nLoS excess path-loss std. dev. \\
		$N_\mathrm{s},N_\mathrm{g}$ & -121dBm, -129dBm  &Sat and terminal noise floor\\
		$W$ & 125kHz, 1MHz  &Uplink and downlink Bandwidth\\
		$\beta$ & 0.7& Parameter of BAAC Algorithm\\
		\hline 
	\end{tabularx}
	\label{Table_Notations}
\end{table}
\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.2]{Figure1.eps} 
\includegraphics[scale=0.2]{Figure6.eps} 
\end{center}
\caption{a) Buffer overflow probabilities, b) Traffic intensities.}
        \label{Fig:Traffic}
\end{figure}
% \begin{figure}[b]
% \begin{center}
% \includegraphics[scale=0.2]{Figure2.eps} 
% \end{center}
% \caption{Queuing delay vs increase in droptail buffer size  with different beamwidth ($\psi_{\mathrm{up}}\in\{30^\circ, 35^\circ, 40^\circ, 45^\circ, 50^\circ\}$).}
%         \label{Fig:Queuing}
% \end{figure}


\section{Results and Discussion}

We first perform the performance evaluation of the developed analytical framework and then discuss the findings and empirical solution of the proposed BAAC algorithm. We create an empirical network setup and implement simulation code in MATLAB for the network scenario and analytic modeling as explained in Figs.~\ref{fig:first},~\ref{fig:block}, and~\ref{Fig_Schematic}. The geometric Monte-Carlo simulator is developed to generate a LEO satellite on a sphere with altitude $R_\oplus + h$ and two independent point processes; (i) uniformly distributed points on a sphere cap representing IoT devices, (ii) ground terminal that is randomly located on the same spherical cap. The coordinates of the uniformly distributed points follow $\vartheta \sim \mathcal{U}(0,2\pi)$ and $\phi \sim \asin[\mathcal{U}(-1,1)]$ for the local elevation and azimuth angles respectively, where $\mathcal{U}(a,b)$ is the uniform random variable between $a$ and $b$. Table~\ref{Table_Notations} summarizes the parameters used for the simulation setup.

%\subsection{Performance Evaluation}

Figs.~\ref{Fig:Traffic} a) and b) demonstrate the effect on the buffer overflow probability and traffic intensity with varying uplink beamwidths (i.e., $\psi_{\mathrm{up}}\in\{30^\circ, 35^\circ, 40^\circ, 45^\circ, 50^\circ\}$). It can be observed in Fig.~\ref{Fig:Traffic} a) that when the arrival rate increases due to the increase in the beamwidth $\psi_{up}$, for the same size droptail buffer $K$, the
$p_{\rm b}$ increases (resp. decreases), as the beadwidth $\psi_{up}$ increases  (resp. decreases). In contrast, the $p_{\rm b}$ decreases with the increase in the size of the droptail buffer. Also, the slope (rate of decrease rate of $p_{\rm b}$) decreases with the increase in $K$. Fig.~\ref{Fig:Traffic} b) demonstrates that, as expected, for the given channel conditions, the traffic intensity increases with increase in the beamwidth $\psi_{up}$, but the fluctuations in the intensity also increases. 

% Fig.~\ref{Fig:Queuing} demonstrates the impact in the queuing delay due to increase in the droptail buffer size for several values of the beamwidth $\psi_{up}$. Observe that the delay increases with an increase in K, but the cumulative effect due to the change in uplink beamwidth on the queuing delay is very small. %In summary, Figs.~\ref{Fig:BufferOverflow},~\ref{Fig:Queuing} and~\ref{Fig:Traffic} validate that the LEO queues can be dynamically adjusted so that the adverse effects of environment and channel variations on the data collection can be balanced by the proportional sharing of packets in the LEO queues. This observation results in improved throughputs and delays of the overall system. As long as the LEO queues are the bottleneck, tuning it will only change distribution across LEOs' queues, based on uplink and downlink channels, therefore, the overall system throughput and delay experience can be improved dynamically.
Observe in Fig.~\ref{Fig:rati} a) the low standing average queues, $\bE[Q_n]$, minimizing queuing delays with BAAC, which is in sharp contrast with the Droptail Queuing (always having near full queue occupancy and high queuing delays). Such an improvement is attainable by adjusting the LEO queues (by tuning $\cR_n$). %Recall that we have used these findings as main presumptions while developing the proposed BAAC algorithm.

\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.2]{FigBACCT1c.eps} 
\includegraphics[scale=0.2]{Figratio.eps} 
\end{center}
\caption{a) Queue occupancy, b) Traffic intensities, with and without BAAC algorithm.}
        \label{Fig:rati}
\end{figure}
\begin{figure}[t]
\begin{center}
\includegraphics[scale=0.19]{Figpb.eps} 
\includegraphics[scale=0.18]{FigTQ.eps} 
\end{center}
\caption{a) Buffer overflow probability, b) Queuing delay, with and without BAAC algorithm.}
        \label{Fig:TQ}
\end{figure}
% \begin{figure}[!h]
% \begin{center}
% \includegraphics[scale=0.4]{instability.pdf} 
% \end{center}
% \caption{There are oscillations in traffic intensity when the system dynamics are unstable. When $\beta K_n=20$, the horizontal dispersion of the black dots, for example, shows the magnitude of the oscillations around an unstable equilibrium point ($\varrho^*, p_b^*$).}
%         \label{Fig:RatEQ}
% \end{figure}
% \begin{figure}[t]
% \begin{center}
% \includegraphics[scale=0.4]{FigRTT.eps} 
% \end{center}
% \caption{Time-varying evolution of End-to-End data collection delay over time with and without BAAC algorithm.}
%         \label{Fig:TQ}
% \end{figure}

%\subsection{With BAAC algorithm}
With extensive simulations we compare the difference of the droptail buffer with that of BAAC at the LEOs. Fig.~\ref{Fig:rati} b) shows that the impact of buffering with BAAC and that of droptail on the traffic intensity $\varrho$ is not noticeable. However, it is quite prevalent in case of buffer overflow loss probabilities and queuing delay, as shown in Fig.~\ref{Fig:TQ} a) and Fig.~\ref{Fig:TQ} b) respectively. In particular, it can be observed in Fig.~\ref{Fig:TQ} a) that the buffer overflow probability becomes more tractable with BAAC, which can be adjusted based on needs. Fig.~\ref{Fig:TQ} b) demonstrates that BAAC mandates low delay due to the low standing queues when compared to the droptail buffers.% Also, with BAAC, the queuing delays are directly adjustable simply by tuning the $0<\beta<1$, which can be used for cooperatively adjusting the fraction of data collections by the participating LEOs (by tuning $\cR_n$). 

% Even with all these potential benefits of BAAC, the effects of buffering at router queues have been recognized in the literature~\cite{mckeown2019sizing} as being quite crucial to the stability of the data collection mechanism. Next, we have included a preliminary instability evaluation of the proposed BAAC algorithm. 

% \subsection{Instability Analysis}

% It's likely that with the proposed BAAC algorithm, the system dynamics may become locally unstable, but the oscillations are not often harmful. To examine this, we plot the amplitude of the oscillations in Fig.~\ref{Fig:RatEQ} for various buffer sizes, using the method described in Sec~\ref{sec:stability}. The magnitude of oscillations is indicated by the horizontal bar around the equilibrium ($\varrho^*, p_b^*$). As shown in Fig.~\ref{Fig:RatEQ}, the system dynamics is not converging for LEO buffer sizes less than roughly $20$ packets. For $\beta K$ = 20 packets, for example, we have highlighted the oscillations and shown their amplitude Fig.~\ref{Fig:RatEQ}. The oscillations are serious when the intensity $\varrho$ is less than unity, which is indicated by the negative infinite values of $log_{10}p_b$. The corresponding evolution of queuing delays and queue occupancy were examined in Fig.~\ref{Fig:RatTQ} and Fig.~\ref{Fig:RatQ} to study the stability and convergence issues. We can clearly observe the gaps and discontinuities in the plots of Fig.~\ref{Fig:RatTQ} and Fig.~\ref{Fig:RatQ}, with the increase in traffic intensity. We take the four cases from Fig.~\ref{Fig:RatEQ} and find the performance to see how severe the oscillations are. We study the performance in terms of $p_b(.)$ and find that the system performance is proportional to \[\varrho^* \times \left(1- p_b\left(\varrho^*\right)\right)\] at a stable equilibrium point $\left(\varrho^*, p_b^*\right)$. 

% At an unstable equilibrium where the traffic intensity oscillates with amplitude $B$ (say), the performance is proportionally fluctuating to the total to
% \[{\frac{1}{2\pi}}{\int_{\theta=0}^{2\pi}\left(\varrho+B \sin \theta\right)}\left(1-p_b\left(\varrho+B \sin \theta\right)\right)
% {\rm d} \theta.\]
% We advocate that the LEO buffer size must be carefully chosen—if it is too small ($p_b$ is high), the performance will be degraded due to large buffer overflows and retrasmissions; if it is too large, 
% the performance will also be degraded due to oscillations (see the increase in the delay fluctuations with higher $\beta K_n$ in Fig.~\ref{Fig:RatTQ}). 



% % \begin{figure}[t]
% % \begin{center}
% % \includegraphics[scale=0.4]{Figratio.eps} 
% % \end{center}
% % \caption{Time-varying traffic intensities comparison with and without BAAC algorithm.}
% %         \label{Fig:TQ}
% % \end{figure}

% \begin{figure}[t]
% \begin{center}
% \includegraphics[scale=0.4]{FigratTQ.pdf} 
% \end{center}
% \caption{Evolution of Queuing delay with traffic intensities as observed in the LEO buffer for the scenario in Fig.~12.}
%         \label{Fig:RatTQ}
% \end{figure}
% \begin{figure}[t]
% \begin{center}
% \includegraphics[scale=0.4]{FigratEQ.pdf} 
% \end{center}
% \caption{Evolution of Queuing occupancy with traffic intensities as observed in the LEO buffer for the scenario in Fig.~12.}
%         \label{Fig:RatQ}
% \end{figure}


\section{Conclusion}
